Non-Parametric Methods Applied to the N-Sample Series Comparison

Anomaly and similarity detection in multidimensional series have a long history and have found practical usage in many different fields such as medicine, networks, and finance. Anomaly detection is of great appeal for many different disciplines; for example, mathematicians searching for a unified mathematical formulation based on probability, statisticians searching for error bound estimates, and computer scientists who are trying to design fast algorithms, to name just a few. In summary, we have two contributions: First, we present a self-contained survey of the most promising methods being used in the fields of machine learning, statistics, and bio-informatics today. Included we present discussions about conformal prediction, kernels in the Hilbert space, Kolmogorov's information measure, and non-parametric cumulative distribution function comparison methods (NCDF). Second, building upon this foundation, we provide a powerful NCDF method for series with small dimensionality. Through a combination of data organization and statistical tests, we describe extensions that scale well with increased dimensionality.

==> abstract.tex <==
Anomaly-and-Similarity detection in multidimensional series has a long
history, it finds practical uses in different fields (i.e., medicine,
networks, and finance), it is of great appeal to mathematicians
searching a unified mathematical formulation, to statisticians
searching for error bound estimates, and to computer scientists for
the design of fast algorithms (for all of the above).

We have two main contributions: First, this work is a self contained
survey of the most promising methods in the fields of machine
learning, statistics and bio-informatics: conformal prediction,
kernels in Hilbert space, Kolmogorov's information measure, and
non-parametric cumulative distribution-function (NCDF) comparison
methods. Second, we provide an original contribution for the latter
(NCDF), in fact, we introduce one of the most powerful methods for
small dimension series and, by a combination of data organization and
statistic tests, we provide extensions that scale well as the series'
dimensions increase.

We shed a new light onto these methods by a clear and complete
exposition of their computation {\em operandi}, we introduce their
theoretical background, we explain their limitations, and we provide
extensive practical experimentation (from synthetic, classified,
research and stock-market series). In practice, we extend the
analysis-tool-set arsenal by a unique methodology and new promising
software tools. 


